Time-Sensitive Networking in IEEE 802.11be: On the Way to Low-latency WiFi 7

Short time after the official launch of WiFi 6, IEEE 802.11 working groups are already designing its successor in the wireless local area network (WLAN) ecosystem: WiFi 7. With the IEEE 802.11be amendment as one of its main constituent parts, future WiFi 7 aims to include time-sensitive networking (TSN) capabilities to support low latency and ultra reliability in license-exempt spectrum bands. This article first introduces the key features of IEEE 802.11be, which are then used as the basis to discuss how TSN functionalities could be implemented in WiFi 7. Finally, benefits and requirements of the most representative low-latency use cases for WiFi 7 are reviewed.

==> RefsTable2.tex <==

% Netflix on video needs
https://help.netflix.com/en/node/306

% VR
https://www.researchgate.net/figure/VR-network-requirements-bandwidth-and-latency_tbl1_319049968

% Per comentar, definició latency
https://medium.com/exmachinagroup/the-ultra-low-latency-video-streaming-roadmap-from-webrtc-to-cmaf-5b0d8b4ceec2

% Impact of latency slide is interesting
https://www.caida.org/workshops/aims/1703/slides/aims1703_mwittie.pdf

%QUalcomm AR
https://www.qualcomm.com/media/documents/files/vr-and-ar-pushing-connectivity-limits.pdf

% VR/AR need 5-8 ms to avoid dizziness
https://5g.co.uk/guides/5g-virtual-reality-and-augmented-reality/
% 20 ms creates nausea
https://www.cmswire.com/digital-workplace/how-5g-will-impact-augmented-and-virtual-reality-use/

% Latency, per rellegir (Marc)
https://ieeexplore-ieee-org.sare.upf.edu/abstract/document/6831322
https://ieeexplore-ieee-org.sare.upf.edu/abstract/document/6123651

% Xbox on gaming requirements
https://support.xbox.com/en-US/xbox-360/networking/slow-performance-solution?kbid=111011&utm_source=highspeedinternet.com&utm_medium=affiliate
https://www.xfinity.com/hub/internet/internet-speed-for-gaming

% Google STadia Requirements (cloud gaming)
https://support.google.com/stadia/answer/9607891?hl=en
gamesradar.com/google-stadia-bandwidth-requirement/

%telesurgery
https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6067812/
%super interessant TAULA 1
https://arxiv.org/pdf/1803.03586.pdf
https://www.ncbi.nlm.nih.gov/pmc/articles/PMC1422462/

%telerehabilitation
https://people.cs.kuleuven.be/~danny.weyns/papers/2017IoT-ASAP.pdf

% Process automation (DOC)
https://www.google.com/url?sa=t&rct=j&q=&esrc=s&source=web&cd=10&ved=2ahUKEwiQ6Ju_nIrmAhUux4UKHTbcBykQFjAJegQIAhAC&url=https%3A%2F%2Fwww.itu.int%2Fdms_pub%2Fitu-r%2Fmd%2F15%2Fwp5a%2Fc%2FR15-WP5A-C-0469!N36!MSW-E.docx&usg=AOvVaw1VSNenbY8ciURtlcZVNHgT

% Process automation (google book) 
https://books.google.es/books?id=yhmIDwAAQBAJ&pg=PA12&lpg=PA12&dq=process+automation+remote+mbps+latency&source=bl&ots=-mzdf0Acio&sig=ACfU3U0b_3K8bMbCZnaqToQnW6uyXWRUmA&hl=en&sa=X&ved=2ahUKEwiQ6Ju_nIrmAhUux4UKHTbcBykQ6AEwAHoECAoQAQ#v=onepage&q=process%20automation%20remote%20mbps%20latency&f=false

% Human Machine Interface
https://www.researchgate.net/publication/317099392_Next_Generation_Industrial_Radio_LAN_for_Tactile_and_Safety_Applications
https://arxiv.org/pdf/1804.07553.pdf

% Haptic
https://tech.fb.com/measuring-the-perception-of-latency-with-a-haptic-glove/
https://www.accenture.com/_acnmedia/pdf-68/accenture-tactile-internet-enabled-pervasive-networks.pdf %taula
https://futurenetworks.ieee.org/images/files/pdf/FirstResponder/Rapeepat-Ratasuk-Nokia.pdf

% Drone
http://www.caac.gov.cn/en/HYYJ/NDBG/201802/P020180227616856973062.pdf
https://arxiv.org/pdf/1803.11048.pdf % taula xula

% Automated Guided Vehicle
https://arxiv.org/pdf/1811.11468.pdf % Unmanned Vehicles Factory
https://futurenetworks.ieee.org/images/files/pdf/FirstResponder/Rapeepat-Ratasuk-Nokia.pdf

% Trading
https://www.cisco.com/c/dam/en_us/solutions/industries/docs/finance/corvil_Latency_mkt_data.pdf




% Per obrir durant el conclave

% Refs Toni
https://ieeexplore.ieee.org/document/8367785
https://ieeexplore.ieee.org/document/8458130
https://arxiv.org/pdf/1808.02079.pdf
%PPT


% Impact of latency
https://www.caida.org/workshops/aims/1703/slides/aims1703_mwittie.pdf
% AR Qualcomm
https://www.qualcomm.com/media/documents/files/vr-and-ar-pushing-connectivity-limits.pdf

%Latencies 
https://arxiv.org/pdf/1803.03586.pdf

% Process automation
https://books.google.es/books?id=yhmIDwAAQBAJ&pg=PA12&lpg=PA12&dq=process+automation+remote+mbps+latency&source=bl&ots=-mzdf0Acio&sig=ACfU3U0b_3K8bMbCZnaqToQnW6uyXWRUmA&hl=en&sa=X&ved=2ahUKEwiQ6Ju_nIrmAhUux4UKHTbcBykQ6AEwAHoECAoQAQ#v=onepage&q=process%20automation%20remote%20mbps%20latency&f=false

% HMI
https://arxiv.org/pdf/1804.07553.pdf

% Haptics figura rara p5
https://www.accenture.com/_acnmedia/pdf-68/accenture-tactile-internet-enabled-pervasive-networks.pdf

% UV
https://arxiv.org/pdf/1811.11468.pdf

% Reliabilities Nokia
https://futurenetworks.ieee.org/images/files/pdf/FirstResponder/Rapeepat-Ratasuk-Nokia.pdf

% AGV
https://arxiv.org/pdf/1804.08273.pdfhttps://arxiv.org/pdf/1803.03586.pdf


